On the notions of facets, weak facets, and extreme functions of the Gomory-Johnson infinite group problem

We investigate three competing notions that generalize the notion of a facet of finite-dimensional polyhedra to the infinite-dimensional Gomory-Johnson model. These notions were known to coincide for continuous piecewise linear functions with rational breakpoints. We show that two of the notions, extreme functions and facets, coincide for the case of continuous piecewise linear functions, removing the hypothesis regarding rational breakpoints. We then separate the three notions using discontinuous examples.

==> Makefile <==
LATEX=latex
PDFLATEX=pdflatex
FIG2DEV=fig2dev
BIBTEX=bibtex

FIGURESDIRPREFIX=

MAINTEXFILE=software-abstract

all: $(MAINTEXFILE).pdf

%.pstex_t: %.fig #Makefile
	$(FIG2DEV) -L pstex_t -p $*.pstex $< $@

%.pstex: %.fig #Makefile
	$(FIG2DEV) -L pstex $< $@

%.pdftex_t: %.fig #Makefile
	$(FIG2DEV) -L pdftex_t -p $*.pdf $< $@

%.pdf: %.fig #Makefile
	$(FIG2DEV) -L pdftex $< $@

SOFTWARE_ABSTRACT_GRAPHICS_SOURCES=

SOFTWARE_ABSTRACT_GENERATED_GRAPHICS=$(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdftex_t) $(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdf) 

#$(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=%.pstex_t) $(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=%.pstex)

SOFTWARE_ABSTRACT_SOURCES=Makefile $(MAINTEXFILE).tex $(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.fig) \
	sage-commands.tex

SOFTWARE_ABSTRACT_STYLES = llncs.cls

## copied these files from their source:
## $ (cd ~/Dropbox/yuan-group-relaxation-sage-code/ && tar cf - $files) | tar xvf -
SOFTWARE_ABSTRACT_GRAPHICS=$(SOFTWARE_ABSTRACT_GENERATED_GRAPHICS)						\
	graphics-for-algo-paper/2d_diagram_with_cones_continuous_deco.png					\
	graphics-for-algo-paper/2d_diagram_with_cones_discontinuous.png						\
	graphics-for-algo-paper/2d_with_cones_discontinuous.png							\
	graphics-for-algo-paper/2d_with_faces_discontinuous.png							\
	graphics-for-algo-paper/construct_a_face.png

# copy-graphics-from-dropbox:
# 	(cd $$HOME/Dropbox/yuan-group-relaxation-sage-code/ && tar cf - $(SOFTWARE_ABSTRACT_GRAPHICS)) | tar xvf -

BIB=../../bib/MLFCB_bib.bib

.PHONY: figures

figures: $(SOFTWARE_ABSTRACT_GRAPHICS) 

$(MAINTEXFILE).pdf: $(MAINTEXFILE).tex $(SOFTWARE_ABSTRACT_GRAPHICS) $(BIB)
	$(PDFLATEX) -halt-on-error "$<"
	$(BIBTEX) $(MAINTEXFILE)
	$(PDFLATEX) -halt-on-error "$<"
	$(PDFLATEX) -halt-on-error "$<"

SOFTWARE_ABSTRACT_SOURCES_AND_MORE=$(SOFTWARE_ABSTRACT_SOURCES) $(SOFTWARE_ABSTRACT_GRAPHICS) $(SOFTWARE_ABSTRACT_STYLES)

.PHONY: arxiv
arxiv:
	COPYFILE_DISABLE=true tar -cf $(CURDIR)/$(MAINTEXFILE).tar	\
		$(MAINTEXFILE).bbl					\
		$(SOFTWARE_ABSTRACT_SOURCES)					\
		$(SOFTWARE_ABSTRACT_GRAPHICS)					\
		$(SOFTWARE_ABSTRACT_STYLES)
	rm -f $(MAINTEXFILE).tar.gz
	gzip $(MAINTEXFILE).tar

